Learning Internal Representations (PhD Thesis)

Most machine learning theory and practice is concerned with learning a single task. In this thesis it is argued that in general there is insufficient information in a single task for a learner to generalise well and that what is required for good generalisation is information about many similar learning tasks. Similar learning tasks form a body of prior information that can be used to constrain the learner and make it generalise better. Examples of learning scenarios in which there are many similar tasks are handwritten character recognition and spoken word recognition. The concept of the environment of a learner is introduced as a probability measure over the set of learning problems the learner might be expected to learn. It is shown how a sample from the environment may be used to learn a representation, or recoding of the input space that is appropriate for the environment. Learning a representation can equivalently be thought of as learning the appropriate features of the environment. Bounds are derived on the sample size required to ensure good generalisation from a representation learning process. These bounds show that under certain circumstances learning a representation appropriate for $n$ tasks reduces the number of examples required of each task by a factor of $n$. Once a representation is learnt it can be used to learn novel tasks from the same environment, with the result that far fewer examples are required of the new tasks to ensure good generalisation. Bounds are given on the number of tasks and the number of samples from each task required to ensure that a representation will be a good one for learning novel tasks. The results on representation learning are generalised to cover any form of automated hypothesis space bias.

==> binfig.tex <==
\begin{figure}
\label{binfig1}
\begin{center}
\leavevmode
\epsfbox{2.eps}
\vspace{1mm}
\epsfbox{6.eps}
\caption{Binary representation generalisation curves ($m=2$ and $m=6$).}
\end{center}
\end{figure}

\begin{figure}
\label{binfig2}
\begin{center}
\leavevmode
\epsfbox{10.eps}
\vspace{30mm}
\epsfbox{18.eps}
\caption{Binary representation generalisation curves ($m=10$ and $m=18$).}
\end{center}
\end{figure}


==> ref.tex <==
\Refs
\ref 
\paper Decision Theoretic Generalizations of the PAC Model for Neural Net
and Other Learning Applications
\by Haussler, D. 
\yr 1992 \vol 100
\jour Inform. Comput.
\pages 78--150
\endref

\ref 
\book Introduction to Statistical Inference
\by Keifer, J.C 
\publ Springer-Verlag
\publaddr New York 
\yr 1987
\endref

\ref
\paper A theory of the learnable
\by Valiant, L.G
\yr 1984 \vol 27 \issue 11
\pages 1134--1142
\jour Comm. ACM
\endref

\ref 
\paper Central limit theorems for empirical measures
\by Dudley, R.M. 
\yr 1978 \vol 6 \issue 6 \pages 899--929
\jour Ann Probab.
\endref

\ref 
\paper A course on empirical processes 
\by Dudley, R.M.
\inbook Lecture Notes in Mathematics
\vol 1097 \pages 2--142 \yr 1984
\publ Springer-Verlag
\publaddr New York
\endref

\ref
\book Convergence of Stochastic Processes
\by Pollard, D.
\yr 1984
\publ Springer-Verlag
\publaddr New York
\endref

\ref
\book Empirical processes: Theory and Applications
\by Pollard D.
\yr 1990
\bookinfo NSF-CBMS Regional Conference Series in Probability and Statistics, 
Vol. 2, Inst. of Math. Stat. and Am. Stat. Assoc.
\endref

\ref
\book Estimation of Dependencies Based on Empirical Data
\by Vapnik, V.
\yr 1982
\publ Springer-Verlag
\publaddr New York
\endref

\ref
\paper On the uniform convergence of relative frequencies of events to their
probabilities
\by Vapnik, V.N. and Chervonenkis, A. YA.
\yr 1971 \vol 16 \issue 2 \pages 264--280
\jour Theory Probab. Appl. 
\endref

\ref
\paper Neural Networks and the Bias/Variance Dilemma
\by Geman S., Bienenstock E. and Doursat R.
\yr 1992 \vol 4 \issue 1 \pages 1--58
\jour Neur. Comp. 
\endref

